A cut finite element method for the Darcy problem

We present and analyze a cut finite element method for the weak imposition of the Neumann boundary conditions of the Darcy problem. The Raviart-Thomas mixed element on both triangular and quadrilateral meshes is considered. Our method is based on the Nitsche formulation studied in [10.1515/jnma-2021-0042] and can be considered as a first attempt at extension in the unfitted case. The key feature is to add two ghost penalty operators to stabilize both the velocity and pressure fields. We rigorously prove our stabilized formulation to be well-posed and derive a priori error estimates for the velocity and pressure fields. We show that an upper bound for the condition number of the stiffness matrix holds as well. Numerical examples corroborating the theory are included.

==> Sections/burman.tex <==
Let $V_h\times Q_h$ be the Raviart-Thomas isogeometric element. Let us impose an extra constraint in order to filter out constant pressures:
\begin{equation*}
Q_I:=\{q_h\in Q_h: \int_{\Omega_{\mathcal T_I}}q_h=0\}.
\end{equation*}
where $\Omega_{\mathcal T_I}:=\Omega_{\mathcal T}\setminus \bigcup_{\Gamma_K\ne\emptyset}{K}$. Then, let us stabilize the whole pressure space:
\begin{equation*}
R_h\left(Q_I\right):=\{R_h\left(q_h\right): q_h\in Q_I\}.
\end{equation*}


Find $\left(\u_h,p_h\right)\in V_h\times R_h\left(Q_I\right)$ such that
\begin{equation}\label{burman_prob}
\begin{cases}
a_h(\u_h,\v_h)-&b_1(\v_h,p_h)= \int_{\Omega}\f\cdot \v_h\qquad\forall\ \v_h\in V_h \\
&b_0(\u_h,q_h)= 0\qquad\forall\ q_h\in R_h\left(Q_I\right),
\end{cases}
\end{equation}
where
\begin{equation*}
\begin{aligned}
a_h(\u_h,\v_h)&:=\int_{\Omega} D\u_h : D\v_h -\int_{\Gamma} R_h(\u_h)\cdot\v_h-\int_{\Gamma} \u_h\cdot R_h(\v_h) + \beta\int_{\Gamma}h^{-1}\u_h\cdot\v_h \\
b_m(\v_h,q_h)&:=\int_{\Omega}q_h\dive \v_h -m\int_{\Gamma}q_h\left(\v_h\cdot\n\right)\qquad m\in\{0,1\}
\end{aligned}
\end{equation*}
In order to prove stability, let us follow the following strategy. Fix $\left(\v_h,q_h\right)\in V_h\times R_h\left(Q_I\right)$. We need to construct/find $\left(\w_h,p_h\right)\in V_h\times R_h\left(Q_I\right)$ such that
\begin{enumerate}
\item $\norm{\left(\v_h,q_h\right)}^2\le C_1 \mathcal A\left(\left(\v_h,q_h\right),\left(\w_h,p_h\right) \right)$
\item $\norm{\left(\w_h,p_h\right)}\le C_2\norm{\left(\v_h,q_h\right)}$	
\end{enumerate}	


\begin{lemma}
\begin{equation}\label{1.4}
\frac{\alpha}{2}\norm{\u_h}^2_{1,h}-\frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}\le a_h(\u_h,\u_h)-b_1(\u_h,p_h)+b_0(\u_h,p_h)
\end{equation}	
\end{lemma}	
\begin{proof}
Let $\left(\u_h,p_h\right)\in V_h\times R_h\left(Q_I\right)$ be the solution to~\eqref{burman_prob}. Using Cauchy-Schwarz, the stability property of $R_h$ and Young's inequality with $\varepsilon:=\alpha$:
\begin{equation*}
\begin{aligned}
\abs{-b_1(\u_h,p_h)+b_0(\u_h,p_h)}\le& \norm{h^{\frac{1}{2}}p_h}_{L^2(\Gamma)}\norm{h^{-\frac{1}{2}}\u_h}_{L^2(\Gamma)}\le  C_S\norm{p_h}_{L^2(\Omega_{\mathcal T_I})}\norm{\u_h}_{1,h} \\
\le & \frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}+\frac{\alpha}{2}\norm{\u_h}^2_{1,h}.
\end{aligned}
\end{equation*}
Hence,
\begin{equation*}
 -\frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}-\frac{\alpha}{2}\norm{\u_h}^2_{1,h}\le-b_1(\u_h,p_h)+b_0(\u_h,p_h).
\end{equation*}
By coercivity $\alpha\norm{\u_h}^2_{1,h}\le a_h(\u_h,\u_h)$, so
\begin{equation*}
\frac{\alpha}{2}\norm{\u_h}^2_{1,h}-\frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}\le a_h(\u_h,\u_h)-b_1(\u_h,p_h)+b_0(\u_h,p_h).
\end{equation*}
\end{proof}	

\begin{lemma}
	\begin{equation}\label{1.5}
	\frac{1}{2}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}-\frac{C_I^2}{2}\norm{\u_h}^2_{1,h}\le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation}	
\end{lemma}	
\begin{proof}
Given $p_h\in R_h\left( Q_h\right)$, in particular $\restr{p_h}{\Omega_{\mathcal T_I}}\in L^2_0(\Omega_{\mathcal T_I})$, there exists $\v_p\in \left[H_0^1\left(\Omega_{\mathcal T_I}\right)\right]^2$ such that
\begin{equation}
\begin{cases}
-\dive \v_{p} &= \restr{p_h}{\Omega_{\mathcal T_I}} \quad\text{in}\;\Omega_{\mathcal T_I} \\
 \v_{p}\cdot\n &= 0 \quad\text{on}\;\partial\Omega_{\mathcal T_I} 
\end{cases}
\end{equation}
Burman says $\v_{p,h}:=\pi_{V_h}\v_p\in \left[H_0^1\left(\Omega_{\mathcal T_I}\right)\right]^2\cap V_h$. In particular it holds
\begin{equation}
-\dive \v_{p,h} = p_h \quad\text{in}\;\Omega_{\mathcal T_I},\; \norm{D \v_{p,h}}_{L^2(\Omega)}\le C_I \norm{p_h}_{L^2(;\Omega_{\mathcal T_I})}
\end{equation}
Let $\u_h$ be the solution for the velocity field. Since using $\restr{\v_{p,h}}{\Gamma}=0$
\begin{equation*}
\abs{a_h(\u_h,\v_{p,h})}\le \norm{D \u_h}_{L^2(\Omega_{\mathcal T_I})}\norm{D \v_{p,h}}_{L^2(\Omega_{\mathcal T_I})}
\end{equation*}	
By Young's inequality
\begin{equation*}
a_h(\u_h,\v_{p,h})\ge -\frac{1}{2\eps} \norm{D \u_h}^2_{L^2(\Omega_{\mathcal T_I})}-\frac{\eps}{2}\norm{D \v_{p,h}}^2_{L^2(\Omega_{\mathcal T_I})}
\end{equation*}	
Again, since $\restr{\v_{p,h}}{\Gamma}=0$
\begin{equation*}
-b_1(\v_{p,h},p_h)= \norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}.
\end{equation*}	
So,
\begin{equation*}
-\frac{1}{2\eps} \norm{D \u_h}^2_{L^2(\Omega_{\mathcal T_I})}-\frac{\eps}{2}\norm{D \v_{p,h}}^2_{L^2(\Omega_{\mathcal T_I})}+\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} \le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation*}
Using $ \norm{D \v_{p,h}}_{L^2(\Omega)}\le C_I \norm{p_h}_{L^2(;\Omega_{\mathcal T_I})}$
\begin{equation*}
-\frac{1}{2\eps} \norm{D \u_h}^2_{L^2(\Omega_{\mathcal T_I})}+\left(1-\frac{\eps C_I^2}{2}\right)\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} \le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation*}
Choose $\eps>0$ such that $1-\frac{\eps C_I^2}{2}=\frac{1}{2}$, i.e. $\eps = \frac{1}{C_I^2}$, so that
\begin{equation*}
\frac{1}{2}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} - \frac{C_I^2}{2}  \norm{D \u_h}^2_{L^2(\Omega_{\mathcal T_I})}\le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation*}
Using $\norm{D \u_h}_{L^2(\Omega_{\mathcal T_I})}\le \norm{\u_h}_{1,h}$
\begin{equation*}
\frac{1}{2}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} - \frac{C_I^2}{2}  \norm{\u_h}^2_{1,h}\le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation*}
\end{proof}	

\begin{lemma}
\begin{equation*}
\frac{\alpha}{2}\norm{\u_h}^2_{1,h} + \frac{\alpha}{8C_I^2}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} -\frac{C^2}{2\alpha\gamma}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} \le a_h(\u_h,\w_h) - b_1(\w_h,p_h)
\end{equation*}	
\end{lemma}	
\begin{proof}
Let us compute \eqref{1.4}$+\frac{\alpha}{4C_I^2}$\eqref{1.5}:
\begin{equation*}
\begin{aligned}
\frac{1}{2}\frac{\alpha}{4C_I^2}&\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} - \frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}+\frac{\alpha}{2}\norm{\u_h}^2_{1,h}-\frac{C_I^2}{2}\frac{\alpha}{4C_I^2}\norm{\u_h}^2_{1,h}\\
\le& a_h(\u_h,\u_h)-b_1(\u_h,p_h)+b_0(\u_h,p_h) + \frac{\alpha}{4C_I^2}a_h(\u_h,\v_{p,h})-\frac{\alpha}{4C_I^2}b_1(\v_{p,h},p_h)
\end{aligned}
\end{equation*}	
Let us define $\w_h:=\u_h+\frac{\alpha}{4C_I^2}\v_{p,h}$
\begin{equation*}
\begin{aligned}
	\left(\frac{1}{2}\frac{\alpha}{4C_I^2}-\frac{C_S^2}{2\alpha}\right)&\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} +\left(\frac{\alpha}{2}-\frac{C_I^2}{2}\frac{\alpha}{4C_I^2}\right) \norm{\u_h}^2_{1,h}\\
	\le & a_h(\u_h,\w_h)-b_1(\w_h,p_h)+b_0(\u_h,p_h)
\end{aligned}
\end{equation*}	
and we have
\begin{equation*}
\begin{aligned}
\frac{\alpha^2-4C_I^2C_S^s}{8\alpha C_I^2}&\norm{p_h}^2_{L^2(\Omega)}+\left(\frac{3\alpha}{8}-\frac{C_I^2}{2}\frac{\alpha}{4C_I^2}\right) \norm{\u_h}^2_{1,h}\\
\le & a_h(\u_h,\w_h)-b_1(\w_h,p_h)+b_0(\u_h,p_h)
\end{aligned}
\end{equation*}	
Attention, in general $\frac{\alpha^2-4C_I^2C_S^s}{8\alpha C_I^2}$ is negative!
\end{proof}	


==> Sections/introduction.tex <==
\section{Introduction}
Complex models are processed within Computer Aided Design (CAD) tools where several geometric manipulations are possible. Geometries are described as collection of their boundary surfaces, often defined as tensor-product splines or NURBS, and during the design process these surfaces can be joined, intersected or simply superflous parts can be cut away. All these Boolean operations act on the original surfaces through a common procedure of trimming. When part of a surface is cut away by trimming, the visualization of the geometric object in CAD tools is adapted, but the mathematical description of the surface, \textcolor{magenta}{given by the original surface along with the trimming curves}, remains. This description of the geometry is called ``boundary representation'' (B-rep), and we defer the interested reader to~\cite{piegl_ten_2005,Stroud2006}, or to the recent review~\cite{Marussig2017} and references therein. This representation is clearly not well suited for the simulation of partial differential equations (PDEs).

Several efforts have been undertaken in the last years to improve the usability of CAD geometries in the solution of PDEs, especially after the advent of Isogeometric Analysis (IGA) \cite{Cottrell:2009:IAT:1816404,HUGHES20054135}. Indeed, IGA has been a tremendous success since 2005 with a wide range of applications (see for instance \textcolor{magenta}{the special issue \cite{CMAME-IGA2017}}), and it is becoming a \textcolor{magenta}{mature method}: its mathematical analysis is now well understood~\cite{buffa}, fast assembly and solvers exist today \cite{MR3761002,MR3811621} and strategies for adaptive refinement with a sound mathematical theory are now available, see \cite{1078-0947_2019_1_241} and the references therein. The geometric modelling community has also provided important inputs to this scientific challenge \cite{Cohen15}, and new strategies to define geometric entities through the volume they occupy instead of their boundaries are now emerging, for instance, the volumetric representations (V-reps) proposed in \cite{Massarwi}. On the other hand, trimming remains a main tool for the design of complex models via Boolean operations, and basically all developments of IGA described above rely on strong requirements on the underlying geometric models and, in general, do not support trimmed geometric entities. The aim of this paper is to contribute to the design of isogeometric methods that robustly support trimming in the geometric description of the computational domain, and do not require the construction of a global re-parametrization (meshing).


The two main issues arising when dealing with trimmed geometries are the presence of elements unfitted with the boundary, making the research for efficient quadrature rules and the stable imposition of boundary conditions a challenge, and the existence of basis functions whose support has been cut, affecting the conditioning of the related linear system. In this regard, ideas from fictitious domain and immersed boundary approaches in the FEM literature can be adapted to the IGA setting, and the related engineering literature includes (but is not limited to) the pioneering works regarding the integration with CAD and numerical quadrature~\cite{NAGY2015165,Wang2015}, the shell analysis on geometric models with B-reps \cite{BREITENBERGER2015401,PHILIPP2016312}, and the finite cell method combined with IGA \cite{Dauge2015,RANK2012104,MR3003066,MR3706626}. \textcolor{magenta}{I would remove \cite{Dauge2015} (it is $p$-FEM)} Concerning the lack of stability, we should mention stabilizations based on extrapolation \cite{ doi:10.1137/S0036142900373208,MARUSSIG201879}, and the Cut-IGA method proposed in \cite{1812.08568}, which is related to the many contributions of Cut-FEM and ghost penalty methods \cite{BURMAN20101217,NME:NME4823,BURMAN2012328,Burman2012,Hansbo434217}.

We now describe the simplified mathematical setting. Let $\Omega_0\subseteq \R^d$ (here $d=2,3$)  be a domain described by a bijective spline map $\mathbf{F}: (0,1)^d \to \Omega_0$, i.e., a patch in the isogeometric terminology, and let $\Omega_1,\ldots \Omega_N$ be Lipschitz regular domains in $\R^d$. We assume that $\bigcup_{i=1}^N\overline{\Omega}_i$ are to be cut away from $\Omega_0$ and that our computational domain reads:  
\begin{equation}\label{48}
\Omega=\Omega_0\setminus\bigcup_{i=1}^N\overline{\Omega}_i.
\end{equation}
After trimming the mathematical description of the domain remains unchanged, that is, the elements and basis functions fit the boundary of $\Omega_0$ instead of that of $\Omega$. In this paper, we focus on a simple Poisson problem, with weakly imposed boundary conditions, on the domain $\Omega$ described above. First of all, we discuss the difference between bad matrix conditioning and lack of stability. The first one can be improved by modifying the chosen basis (preconditioning), while the second one needs to act on the bilinear form directly. 

Regarding the lack of stability, we propose a minimal stabilization technique, inspired by \cite{Renard}, that acts only on those cut elements that affect stability. For example, in the case of a Neumann condition on the trimmed boundary, no stabilization is needed. Our stabilization is parameter free, and its computation requires only local projections at the element level, and only for  ``bad'' cut elements. For the stabilization we follow a ``local approach'' (according to the review paper \cite{Marussig2017}), i.e. we modify the analysis, rather than the geometry, in order to be able to face the challenges arising from trimming. We present two different versions of the stabilization technique. The first one in the parametric domain, easier to implement from the numerical point of view, but suboptimal. The second , a projection-based stabilization performed directly on the physical domain, which allows us to recover optimal a priori error estimates.

Concerning the bad conditioning of the matrix, we show numerical evidence that a rescaling of the stiffness matrix seems to consistently  resolve the issue. However, the analysis on the linear algebra side is not presented, as it is beyond the scope of this work.

The document is organized as follows. Section \ref{4} presents an overview of isogeometric analysis in trimmed domains. In Section \ref{35} we set the model problem, and explain the main challenges we need to face, namely integration, conditioning and numerical stability of the associated linear system. %An exhaustive discussion about the issues of integration and conditioning is beyond the scope of this work.
After having explained in detail in Section \ref{section_stability} the causes for the lack of stability of the simple Nitsche's formulation, in Section \ref{36} we present our new stabilization technique. Two possible constructions of the stabilization operator are suggested and analysed in Section~\ref{sec:construction}, and error estimates are provided in Section~\ref{sec:estimate}. 
Finally, we conclude by showing some numerical examples, obtained using the MATLAB library GeoPDEs \cite{VAZQUEZ2016523}, confirming the theoretical results.


%Complex models are processed within Computer Aided Design (CAD) tools where several geometric manipulations are possible. One procedure that is  basically ubiquitous is \emph{trimming}. Geometries are described as collection of  surfaces that can be joined, intersected or simply superflous parts can be cut away. Often surfaces are bivariate splines or NURBS surfaces and this representation is called ``boundary representation'' (B-rep).  We defer the interested reader to \cite{piegl_ten_2005,Stroud2006}, or to the recent review \cite{Marussig2017} and the references there in. 

%When superflous parts are cut away, the geometric object changes but its mathematical description does not. Clearly this representation is not well suited for the simulation of PDEs and, as a matter of fact, several efforts have been undertaken in the last years to improve the usability of CAD geometries in analysis, especially after the advent of Isogeometric Analysis (IGA) \cite{Cottrell:2009:IAT:1816404,HUGHES20054135}. Indeed, since 2005, also the geometric modelling community has provided important inputs to this scientific challenge \cite{Cohen15} and new strategies to define geometric entities through the volume they occupy instead of their boundaries are now emerging. For instance, in \cite{Massarwi} volumetric representations (V-reps) are proposed as a new, more analysis friendly, geometric design paradigm. On the other hand, trimming remains a main tool allowing for the design of complex models via Boolean operations (such as union, intersection, difference). Thus, in order to guarantee interoperability, in the spirit of isogeometric analysis, we wish to  design tools for the approximation of PDEs that support trimming in the geometric description of the computational domain and do not require the construction of global re-parametrization (meshing). 

%Indeed, isogeometric analysis has been a tremendous success since 2005. It has been successfully applied to many problems, from elasticity \cite{laura18b,MR3610117,Cottrell:2009:IAT:1816404,laura14,MR3196811}, to phase fields models \cite{MR3527591}, to fracture analysis \cite{laura16}, to electromagnetics \cite{mio2,mio1}; its mathematical analysis is now well understood \cite{buffa}, fast assembly and solvers exist today \cite{MR3761002,MR3811621} and strategies for local refinements are now well understood, also from a mathematical stand point e.g., \cite{1078-0947_2019_1_241} and the references therein. This list could continue long.


%On the other hand, basically all developments described above rely on strong requirements on the underlying geometric models and, in general, do not support trimmed geometric entities. The aim of this paper is to contribute to the design of isogeometric methods that robustly support  the use of trimmed geometries.   

%We consider the following simplified situation. Let $\Omega_0\subseteq \R^d$   (here $d=2,3$)  be a domain described by a bijective spline map $\mathbf{F}: (0,1)^d \to \Omega_0$, i.e., a patch in the isogeometric terminology and let $\Omega_1,\ldots \Omega_N$ be Lipschitz regular domains in $\R^d$. We assume that $\bigcup_{i=1}^N\overline{\Omega}_i$ are to be cut away from $\Omega_0$ and that our computational domain reads:  
%\begin{equation}\label{48}
%\Omega=\Omega_0\setminus\bigcup_{i=1}^N\overline{\Omega}_i. 
%\end{equation}
%Let us put ourselves in a situation in which we want to numerically approximate a PDE in a computational domain of the type \eqref{48}. 
%When the superfluous surface areas are cut away, the mathematical description of the domain remains unchanged. It turns out that we have to deal with elements unfitted with the boundary, making the research for efficient quadrature rules and the imposition of boundary conditions a challenge. Moreover there are basis functions, whose support has been cut, affecting the conditioning of the related linear system. In this regard, ideas from fictitious domain and immersed boundary approaches in the FEM literature come to help.

%Indeed, the related engineering literature includes (but is not limited to) the pioneering work  \cite{NAGY2015165,Wang2015} or \cite{BREITENBERGER2015401,PHILIPP2016312} for shell analysis and the finite cell method \cite{Dauge2015,RANK2012104,MR3003066,MR3706626}. 

%In order to guarantee robustness, some stabilization is needed, and our work is related to the previous contributions in this context. In particular, we should mention stabilizations based on extrapolation \cite{ doi:10.1137/S0036142900373208,MARUSSIG201879}, and the Cut-Iga method proposed in \cite{1812.08568},  which is related to the many contributions \cite{BURMAN20101217,NME:NME4823,BURMAN2012328,Burman2012,Hansbo434217}.

%In this paper, we focus on a simple Poisson problem on the domain $\Omega$ described above, with weakly imposed boundary conditions. First of all, we discuss the difference between bad matrix conditioning and lack of stability. The first one can be improved by modifying the chosen basis (preconditioning), while the second one needs to act on the bilinear form directly. 

%Regarding the lack of stability, we propose a minimal stabilization technique, inspired by \cite{Renard}, that acts only on those cut elements that generate the lack of stability. For example, in the case of Neumann boundary condition on the trimmed boundary, no stabilization is needed. Our stabilization is parameter free, and its computation requires only local projections at the element level, and only for  ``bad'' cut elements. For the stabilization we follow a ``local approach'' (according to the review paper \cite{Marussig2017}), i.e. we modify the analysis, rather than the geometry, in order to be able to face the challenges arising from trimming. We present two different versions of the stabilization technique. One in the parametric domain, easier to implement from the numerical point of view and, in our opinion, more ``natural'', but suboptimal. The other in the physical domain, a projection-based stabilization, which allows us to recover optimal a priori error estimates.

%Concerning the bad conditioning of the matrix, we show numerical evidence that a rescaling of stiffness matrix seems to consistently  resolve the issue. However, the analysis on the linear algebra side is not presented, as it is beyond the scope of this work. 

%We propose a minimal stabilization technique, inspired by \cite{Renard}, that acts only on those cut elements that generate lack of stability, and leave all issues concerning bad conditioning to a further analysis on the linear algebra side. For example, in the case of Neumann boundary condition on the trimmed boundary, no stabilization is needed. Our stabilization is parameter free, and its computation requires only local projections at the element level, and only for  ``bad'' cut elements.  Moreover, a rescaling of stiffness matrix seems to consistently  resolve the issue of bad conditioning. 

%The document is organized as follows. Section \ref{4} presents an overview of isogeometric analysis in trimmed domains. In Section \ref{35} we set the model problem, the Poisson equation in a trimmed domain, and explain the main challenges we need to face, namely integration, conditioning and numerical stability of the associated linear system. An exhaustive discussion about the issues of integration and conditioning is beyond the scope of this work.
%After having explained in detail in Section \ref{section_stability} the causes for the lack of stability of the simple Nitsche's formulation, in Section \ref{36} we present our new stabilization technique. 
%%We follow a ``local approach'' (according to the review paper \cite{Marussig2017}), i.e. we modify the analysis, rather than the geometry, in order to be able to face the challenges arising from trimming. We present two new stabilization techniques. One in the parametric domain, easier to implement from the numerical point of view and, in our opinion, more ``natural'', but suboptimal. The other in the physical domain, a projection-based stabilization, which allow us to recover optimal a priori error estimates.
%Finally, we conclude by showing some numerical examples, obtained using the MATLAB library GeoPDEs \cite{VAZQUEZ2016523}, confirming the theoretical results.

%The document is organized as follows. Section \ref{4} presents an overview of isogeometric analysis in trimmed domains. In Section \ref{35} we set the model problem, the Poisson equation in a trimmed domain, and explain the main challenges we need to face, namely integration, conditioning and numerical stability of the associated linear system. An exhaustive discussion about the issues of integration and conditioning is beyond the scope of this work.
%After having explained in detail in Section \ref{section_stability} the causes for the lack of stability of the simple Nitsche's formulation, in Section \ref{36} we present our new stabilization. We follow a ``local approach'' (according to the review paper \cite{Marussig2017}), i.e. we modify the analysis, rather than the geometry, in order to be able to face the challenges arising from trimming. We present two new stabilization techniques. One in the parametric domain, easier to implement from the numerical point of view and, in our opinion, more ``natural'', but suboptimal. The other in the physical domain, a projection-based stabilization, which allow us to recover optimal a priori error estimates.
%Finally, we conclude by showing some numerical examples, obtained using the MATLAB library GeoPDEs (\cite{VAZQUEZ2016523}), confirming the theoretical results.
%


==> Sections/numerical_experiments_old.tex <==
\section{Numerical examples}\label{section_numerical_examples}
In the following, we use the ghost penalty projection-based operators defined in Remark~\ref{rmk:ghost_penalty}. This choice is convenient from the implementation point of view since it spares us to calculate the jumps of possibly high-order normal derivatives through the facets in the vicinity with the trimmed boundary. We limit the scope of our numerical investigations to the case of Cartesian quadrilateral meshes in $2$D. The numerical experiments have been carried out in the \textsc{Matlab} library GeoPDEs~\cite{MR3521056}. To perform integration close to the trimming line, we employ the strategy depicted in~\cite{MR3982623}, where the cut elements are reparametrized using polynomials with the same approximation order of the Raviart-Thomas space employed for the space discretization.
\begin{figure}[!ht]
	\centering
	\subfloat[][\emph{Trimmed rectangle}.\label{fig:trimmed_square}]
	{
	\includestandalone[]{mesh_epsilon}
	}
	\subfloat[][\emph{Square with circular hole}.\label{figure:fig5}]
{
	\includestandalone[]{plate_with_hole}
}
\\
	\subfloat[][\emph{Trimmed pentagon}.\label{fig:trimmed_pentagon}]
{
	\includestandalone[]{mesh_epsilon_pentagon}
}
	\subfloat[][\emph{Circle}.\label{figure:fig9}]
	{
	\includestandalone[]{circle}
	}
	\caption{Unfitted domains employed for the numerical experiments.}\label{figure:domains}
\end{figure}

\subsection{Convergence rates}
\subsubsection{Trimmed rectangle}
Let us start by taking as computational domain the \emph{trimmed rectangle} $\Omega = \left(0,1\right) \times \left( 0,0.75+\eps\right)$ where $\eps$ is a ``small'' controlled parameter, see Figure~\ref{fig:trimmed_square}. The reference solutions are
\begin{align*}
\u_{ex}=
\begin{pmatrix}
y\sin(x)\cos(y)\\
-x\sin(y)\cos(x)
\end{pmatrix}
\qquad
p_{ex}= x^3y.
\end{align*}
In the first set of numerical experiments we fix a degree $k\in\{0,1,2\}$, a geometric parameter $\eps\in \{10^{-k}: k=2m+1,\ m=1,\dots,6\}$ and perform dyadic refinement of the mesh size $h$. The approximation errors of the velocity and pressure fields are computed and shown in Figures~\ref{figure:fig1},~\ref{figure:fig2}.


\begin{figure}[!ht]
	\centering
\includestandalone[]{legend_degrees2}  
\\
	\subfloat[][Velocity error, $\eps=10^{-3}$.]
	{
		\includestandalone[]{error_velocity_trimmedsquare_eps3_gp}
	}
	\subfloat[][Pressure error,  $\eps=10^{-3}$.]
	{
		\includestandalone[]{error_pressure_trimmedsquare_eps3_gp}
	} \\
	\subfloat[][Velocity error, $\eps=10^{-5}$.]
{
	\includestandalone[]{error_velocity_trimmedsquare_eps5_gp}
}
\subfloat[][Pressure error,  $\eps=10^{-5}$.]
{
	\includestandalone[]{error_pressure_trimmedsquare_eps5_gp}
} \\
	\subfloat[][Velocity error, $\eps=10^{-7}$.]
{
	\includestandalone[]{error_velocity_trimmedsquare_eps7_gp}
}
\subfloat[][Pressure error,  $\eps=10^{-7}$.]
{
	\includestandalone[]{error_pressure_trimmedsquare_eps7_gp}
} 
\caption{Convergence rates of the errors in the \emph{trimmed rectangle}.}\label{figure:fig1}
\end{figure}

\begin{figure}[!ht]
	\centering
\includestandalone[]{legend_degrees2}  
\\
	\subfloat[][Velocity error, $\eps=10^{-9}$.]
{
	\includestandalone[]{error_velocity_trimmedsquare_eps9_gp}
}
\subfloat[][Pressure error,  $\eps=10^{-9}$.]
{
	\includestandalone[]{error_pressure_trimmedsquare_eps9_gp}
} \\
\subfloat[][Velocity error, $\eps=10^{-11}$.]
{
	\includestandalone[]{error_velocity_trimmedsquare_eps11_gp}
}
\subfloat[][Pressure error,  $\eps=10^{-11}$.]
{
	\includestandalone[]{error_pressure_trimmedsquare_eps11_gp}
} \\
\subfloat[][Velocity error, $\eps=10^{-13}$.]
{
	\includestandalone[]{error_velocity_trimmedsquare_eps13_gp}
}
\subfloat[][Pressure error,  $\eps=10^{-13}$.]
{
	\includestandalone[]{error_pressure_trimmedsquare_eps13_gp}
} 		
\caption{Convergence rates of the errors in the \emph{trimmed rectangle}.}\label{figure:fig2}
\end{figure}


\subsubsection{Trimmed pentagon}
We consider the same reference solutions as in the previous example, but this time in another domain.  Let $\Omega_0=\left(0,1\right)^2$, $\Omega_1$ be the triangle with vertices $(0,0.25+\eps)-(0,1)-(0.75-\eps,1)$ and $\Omega=\Omega_0\setminus \overline\Omega_1$, see Figure~\ref{fig:trimmed_pentagon}. Neumann boundary conditions are imposed on the whole boundary, weakly just on the sides that do not fit the underlying mesh. Let us compute the approximation errors of the velocity and pressure fields for different degrees $k\in\{0,1,2\}$ and geometric parameters $\eps\in \{10^{-k}: k=2m+1,\ m=1,\dots,6\}$, see Figures~\ref{figure:fig3},~\ref{figure:fig4}.

\begin{figure}[!ht]
	\centering
	\includestandalone[]{legend_degrees2}  
	\\
	\subfloat[][Velocity error, $\eps=10^{-3}$.]
	{
		\includestandalone[]{error_velocity_pentagon_eps3_gp}
	}
	\subfloat[][Pressure error,  $\eps=10^{-3}$.]
	{
		\includestandalone[]{error_pressure_pentagon_eps3_gp}
	} \\
	\subfloat[][Velocity error, $\eps=10^{-5}$.]
	{
		\includestandalone[]{error_velocity_pentagon_eps5_gp}
	}
	\subfloat[][Pressure error,  $\eps=10^{-5}$.]
	{
		\includestandalone[]{error_pressure_pentagon_eps5_gp}
	} \\
	\subfloat[][Velocity error, $\eps=10^{-7}$.]
	{
		\includestandalone[]{error_velocity_pentagon_eps7_gp}
	}
	\subfloat[][Pressure error,  $\eps=10^{-7}$.]
	{
		\includestandalone[]{error_pressure_pentagon_eps7_gp}
	} 
	\caption{Convergence rates of the errors in the \emph{trimmed pentagon}.}\label{figure:fig3}
\end{figure}

\begin{figure}[!ht]
	\centering
	\includestandalone[]{legend_degrees2}  
	\\	
	\subfloat[][Velocity error, $\eps=10^{-9}$.]
	{
		\includestandalone[]{error_velocity_pentagon_eps9_gp}
	}
	\subfloat[][Pressure error,  $\eps=10^{-9}$.]
	{
		\includestandalone[]{error_pressure_pentagon_eps9_gp}
	} \\
	\subfloat[][Velocity error, $\eps=10^{-11}$.]
	{
		\includestandalone[]{error_velocity_pentagon_eps11_gp}
	}
	\subfloat[][Pressure error,  $\eps=10^{-11}$.]
	{
		\includestandalone[]{error_pressure_pentagon_eps11_gp}
	} \\
	\subfloat[][Velocity error, $\eps=10^{-13}$.]
	{
		\includestandalone[]{error_velocity_pentagon_eps13_gp}
	}
	\subfloat[][Pressure error,  $\eps=10^{-13}$.]
	{
		\includestandalone[]{error_pressure_pentagon_eps13_gp}
	} 		
	\caption{Convergence rates of the errors in the \emph{trimmed pentagon}.}\label{figure:fig4}
\end{figure}

%\begin{figure}[!ht]
%	\centering
%	\includestandalone[]{legend_degrees2}  
%	\\
%	\subfloat[][Velocity error, $\eps=10^{-3}$.]
%{
%	\includestandalone[]{error_velocity_pentagon_eps3_gp_bis}
%}
%\subfloat[][Pressure error,  $\eps=10^{-3}$.]
%{
%	\includestandalone[]{error_pressure_pentagon_eps3_gp_bis}
%} \\
%	\subfloat[][Velocity error, $\eps=10^{-5}$.]
%	{
%		\includestandalone[]{error_velocity_pentagon_eps5_gp_bis}
%	}
%	\subfloat[][Pressure error,  $\eps=10^{-5}$.]
%	{
%		\includestandalone[]{error_pressure_pentagon_eps5_gp_bis}
%	} \\
%	\subfloat[][Velocity error, $\eps=10^{-7}$.]
%	{
%		\includestandalone[]{error_velocity_pentagon_eps7_gp_bis}
%	}
%	\subfloat[][Pressure error,  $\eps=10^{-7}$.]
%	{
%		\includestandalone[]{error_pressure_pentagon_eps7_gp_bis}
%	} 
%	\caption{Convergence rates of the errors in the \emph{trimmed pentagon} with GP with $h^{0}$.}\label{figure:fig3_bis}
%\end{figure}
%
%\begin{figure}[!ht]
%	\centering
%	\includestandalone[]{legend_degrees2}  
%	\\	
%	\subfloat[][Velocity error, $\eps=10^{-9}$.]
%	{
%		\includestandalone[]{error_velocity_pentagon_eps9_gp_bis}
%	}
%	\subfloat[][Pressure error,  $\eps=10^{-9}$.]
%	{
%		\includestandalone[]{error_pressure_pentagon_eps9_gp_bis}
%	} \\
%	\subfloat[][Velocity error, $\eps=10^{-11}$.]
%	{
%		\includestandalone[]{error_velocity_pentagon_eps11_gp_bis}
%	}
%	\subfloat[][Pressure error,  $\eps=10^{-11}$.]
%	{
%		\includestandalone[]{error_pressure_pentagon_eps11_gp_bis}
%	} \\
%	\subfloat[][Velocity error, $\eps=10^{-13}$.]
%	{
%		\includestandalone[]{error_velocity_pentagon_eps13_gp_bis}
%	}
%	\subfloat[][Pressure error,  $\eps=10^{-13}$.]
%	{
%		\includestandalone[]{error_pressure_pentagon_eps13_gp_bis}
%	} 		
%	\caption{Convergence rates of the errors in the \emph{trimmed pentagon} with GP with $h^{0}$.}\label{figure:fig4_bis}
%\end{figure}



\subsubsection{Square with circular hole}
We consider as domain the \emph{square with circular hole} depicted in Figure~\ref{figure:fig5}, namely $\Omega=\left(0,2\right)^2\setminus B_r(x_0)$, with $x_0=\left(0,0\right)$ and $r=0.52$. The reference solution is
\begin{align*}
\u_{ex}=
\begin{pmatrix}
	\cos(x)\operatorname{sinh}(y)\\
	\sin(x)\operatorname{cosh}(y)
\end{pmatrix}
\qquad
p_{ex}=-\sin(x)\operatorname{sinh}(y)-\left(\cos(1)-1\right)\left(\operatorname{cosh}(1)-1\right).
\end{align*}
We prescribe Dirichlet boundary conditions along $\{(x,y):x=2,\ 0\le y\le 2\}$ and $\{(x,y):0\le x\le 2,\ y=2\}$ and Neumann boundary conditions, weakly, on the remaining part of the boundary.


\begin{figure}[!ht]
	\centering
\includestandalone[]{legend_degrees2}  
\\	
\subfloat[][Velocity error.]
{
	\includestandalone[]{error_velocity_platehole}
}
\subfloat[][Pressure error.]
{
	\includestandalone[]{error_pressure_platehole}
}
\caption{Convergence rates of the errors in the \emph{square with circular hole}.}\label{figure:fig6}
\end{figure}	

%\begin{figure}[!ht]
%	\centering
%	\includestandalone[]{legend_degrees2}  
%	\\	
%	\subfloat[][Velocity error.]
%	{
%		\includestandalone[]{error_velocity_platehole_bis}
%	}
%	\subfloat[][Pressure error.]
%	{
%		\includestandalone[]{error_pressure_platehole_bis}
%	}
%	\caption{Convergence rates of the errors in the \emph{square with circular hole} with GP with $h^0$.}\label{figure:fig6_bis}
%\end{figure}	

\subsubsection{Circle}
We consider $\Omega= B_r(x_0)$, with $x_0=\left(0.5,0.5\right)$ and $r=0.45$, see Figure~\ref{figure:fig9}. The reference solution for the pressure is
\begin{align*}
p_{ex}=\sin \left( 2\pi x \right) \cos \left( 2\pi \right), 
\end{align*}
and the velocity field is computed from Darcy's law~\eqref{prob:cont} in which $\f$ is taken to be zero. We weakly prescribe Neumann boundary conditions on the whole boundary, which does not fit with the underlying mesh. The $L^2$-errors for the velocity and pressure fields are plotted in Figure~\ref{figure:fig11}.

\begin{figure}[!ht]
	\centering
	\includestandalone[]{legend_degrees2}  
	\\	
	\subfloat[][Velocity error.]
	{
		\includestandalone[]{error_velocity_circle}
	}
	\subfloat[][Pressure error.]
	{
		\includestandalone[]{error_pressure_circle}
	}
	\caption{Convergence rates of the errors in the \emph{circle}.}\label{figure:fig11} 
\end{figure}	



\subsection{Condition number}
\subsubsection{Square with circular hole}
\begin{figure}[!ht]
	\centering
	\includestandalone[]{legend_condnumb}  
	\\	
	\subfloat[][$k=0$.]
	{
		\includestandalone[]{condnumb_platehole_k=0}
	}
	\subfloat[][$k=1$.]
	{
		\includestandalone[]{condnumb_platehole_k=1}
	}\\
	\subfloat[][$k=2$.]
	{
		\includestandalone[]{condnumb_platehole_k=2}
	}
	\subfloat[][$k=3$.]
	{
		\includestandalone[]{condnumb_platehole_k=3}
	}
	\caption{Condition number for the \emph{square with circular hole} with Neumann boundary conditions.}\label{figure:fig8}
\end{figure}	

\begin{figure}[!ht]
	\centering
	\includestandalone[]{legend_condnumb}  
	\\	
	\subfloat[][$k=0$.]
	{
		\includestandalone[]{condnumb_platehole_k=0_dirichlet}
	}
	\subfloat[][$k=1$.]
	{
		\includestandalone[]{condnumb_platehole_k=1_dirichlet}
	}\\
	\subfloat[][$k=2$.]
	{
		\includestandalone[]{condnumb_platehole_k=2_dirichlet}
	}
	\subfloat[][$k=3$.]
	{
		\includestandalone[]{condnumb_platehole_k=3_dirichlet}
	}
	\caption{Condition number for the \emph{square with circular hole} with Dirichlet boundary conditions.}\label{figure:fig8_dirichlet}
\end{figure}	
Let us consider as domain the \emph{square with circular hole} depicted in Figure~\ref{figure:fig5}, namely $\Omega=\left(0,2\right)^2\setminus B_r(x_0)$, with $x_0=\left(0,0\right)$ and $r=0.52$. We prescribe Dirichlet boundary conditions along $\{(x,y):x=2,\ 0\le y\le 2\}$ and $\{(x,y):0\le x\le 2,\ y=2\}$ and Neumann boundary conditions, weakly, on the remaining part of the boundary. We compute the condition number of the linear system arising from~\eqref{cutfem:disc_pb} and compare the cases when we stabilize and when we do not stabilize; see Figure~\ref{figure:fig8}. Then, we impose Dirichlet boundary conditions on the whole boundary and compare the conditioning with the stabilized formulation~\eqref{dirichlet:pb2_stab} and non-stabilized formulation~\eqref{dirichlet:pb2}; see Figure~\ref{figure:fig8_dirichlet}. The results are in agreement with the theory developed in Section~\ref{section:cond_numb}. In particular, we observe that without stabilization, the condition number is negatively affected by the presence of cut elements, while in the stabilized case, the expected scaling of the conditioning is restored.



\subsubsection{Trimmed rectangle}
\begin{figure}[!ht]
	\centering
	\includestandalone[]{legend_condnumb}  
	\\	
	\subfloat[][$k=0$.]
	{
		\includestandalone[]{condnumb_trimmedsquare_k=0}
	}
	\subfloat[][$k=1$.]
	{
		\includestandalone[]{condnumb_trimmedsquare_k=1}
	}\\
	\subfloat[][$k=2$.]
	{
		\includestandalone[]{condnumb_trimmedsquare_k=2}
	}
	\subfloat[][$k=3$.]
	{
		\includestandalone[]{condnumb_trimmedsquare_k=3}
	}
	\caption{Condition number for the \emph{trimmed rectangle} with $\eps=10^{-7}$ with Neumann boundary conditions.}\label{figure:fig80}
\end{figure}
\begin{figure}[!ht]
	\centering
	\includestandalone[]{legend_condnumb}  
	\\	
	\subfloat[][$k=0$.]
	{
		\includestandalone[]{condnumb_trimmedsquare_k=0_dirichlet}
	}
	\subfloat[][$k=1$.]
	{
		\includestandalone[]{condnumb_trimmedsquare_k=1_dirichlet}
	}\\
	\subfloat[][$k=2$.]
	{
		\includestandalone[]{condnumb_trimmedsquare_k=2_dirichlet}
	}
	\subfloat[][$k=3$.]
	{
		\includestandalone[]{condnumb_trimmedsquare_k=3_dirichlet}
	}
	\caption{Condition number for the \emph{trimmed rectangle} with $\eps=10^{-7}$ with Dirichlet boundary conditions.}\label{figure:fig80_dirichlet}
\end{figure}
Let us consider as physical domain the \emph{trimmed rectangle} of Figure~\ref{fig:trimmed_square} with $\eps=10^{-7}$. We impose Neumann boundary conditions weakly on the whole boundary. In Figure~\ref{figure:fig80} we compare the conditioning of the stabilized and non-stabilized formulations. Similarly, in Figure~\ref{figure:fig80_dirichlet} we compare the conditioning of the stabilized and non-stabilized formulations when Dirichlet boundary conditions are imposed.



	


%\begin{figure}[!ht]
%	\centering
%	\includestandalone[]{legend_condnumb}  
%	\\	
%	\subfloat[][$k=0$.]
%	{
%		\includestandalone[]{condnumb_platehole_k=0_bis}
%	}
%	\subfloat[][$k=1$.]
%	{
%		\includestandalone[]{condnumb_platehole_k=1_bis}
%	}\\
%	\subfloat[][$k=2$.]
%	{
%		\includestandalone[]{condnumb_platehole_k=2_bis}
%	}
%	\subfloat[][$k=3$.]
%	{
%		\includestandalone[]{condnumb_platehole_k=3_bis}
%	}
%	\caption{Condition number for the \emph{square with circular hole} with GP $h^{0}$.}\label{figure:fig8_bis}
%\end{figure}	

\subsection{Scaling of Nitsche's parameter}
\subsubsection{Circle}
\begin{figure}[!ht]
	\centering
	\includestandalone[]{legend_gamma}  
	\\	
	\subfloat[][Velocity error.]
	{
		\includestandalone[]{error_velocity_circle_gamma}
	}
	\subfloat[][Pressure error.]
	{
		\includestandalone[]{error_pressure_circle_gamma}
	}
	\caption{Compare $L^2$-errors for different values of the Nitsche parameter in the \emph{circle}.}\label{figure:fig13} 
\end{figure}	
We consider $\Omega= B_r(x_0)$, with $x_0=\left(0.5,0.5\right)$ and $r=0.45$, see Figure~\ref{figure:fig9}. The reference solution for the pressure is $p_{ex}=\sin \left( 2\pi x \right) \cos \left( 2\pi \right)$, and the velocity field is computed from Darcy's law~\eqref{prob:cont} in which $\f$ is taken to be zero. We weakly prescribe Neumann boundary conditions on the whole boundary, which does not fit with the underlying mesh. 

Let us refer to the Nitsche penalty parameter as $\gamma$. So far we have been considering $\gamma:=h^{-1}$, see formulation~\eqref{cutfem:disc_pb}. We observe that the natural space for the Neumann datum is $H^{-\frac{1}{2}}(\Gamma_N)$ and the natural weight to impose the Neumann boundary conditions weakly should mimic the $H^{-\frac{1}{2}}$-norm. This would correspond to add to the Dirichlet energy of the problem the term $\gamma \norm{\u_h\cdot\n-u_N}^2_{L^2(\Gamma_N)}$, with $\gamma:=h$. Thus, it is natural to test the accuracy of our method for different scaling behaviors of $\gamma$, see Figure~\ref{figure:fig13}.


\subsection{On mass conservation}\label{numerical_experiment:mass}
Mass conservation is an important feature for finite element discretizations of incompressible flows, whose violation is not tolerable in many applications~\cite{MR3561143}. As observed in Remark~\ref{remark:mass_conservation}, the Raviart-Thomas mixed element satisfies $\dive V_h =Q_h$ in the unfitted configuration as well. To exploit this property when the right-hand side $g\equiv 0$, we consider the following non-symmetric variant of formulation~\eqref{cutfem:disc_pb}.
	
Find $\left( \u_h,p_h\right) \in V_h\times Q_h$ such that
\begin{equation}\label{cutfem:disc_pb_nonsym}
	\begin{aligned}	
		a_h(\u_h,\vv_h) +  b_1 (\vv_h,p_h) +j_h^v(\u_h,\vv_h)  = \int_\Omega \f\cdot \vv_h + \int_{\Gamma_D} p_D \vv_h\cdot\n + h^{-1} \int_{\Gamma_N} u_N  \vv_h\cdot\n, \qquad &\forall\ \vv_h\in V_h, \\
		b_0 (\u_h,q_h) +j_h^p(p_h,q_h)  = \int_\Omega g q_h,\qquad & \forall\ q_h\in Q_h,
	\end{aligned}
\end{equation}
where
\begin{align*}
	b_0(\w_h,q_h):= \int_\Omega q_h \dive \w_h,\qquad \w_h\in V_h, q_h\in Q_h.
\end{align*}
	
Let us test formulation~\eqref{cutfem:disc_pb_nonsym} in the stabilized and non-stabilized cases.
	
We take as reference solutions
\begin{align*}
	\u_{ex}=
	\begin{pmatrix}
		\cos(x)\operatorname{sinh}(y)\\
		\sin(x)\operatorname{cosh}(y)
	\end{pmatrix}
	\qquad
	p_{ex}=-\sin(x)\operatorname{sinh}(y)-\left(\cos(1)-1\right)\left(\operatorname{cosh}(1)-1\right).
\end{align*}
Note that $g=\dive \u_h = \equiv 0$. We impose Dirichlet boundary conditions on $\{(x,y):x=2, 0\le y\le 2\}$ and on $\{(x,y) : 0\le x\le 2, y=2\}$, and weak Neumann boundary conditions on the rest of the boundary. The computed divergence of the discrete solution for the velocity is shown in Figure~\ref{figure:div_plate}. We observe that the ghost penalty stabilization pollutes the divergence the velocity. 

A possible way to mitigate the loss of preservation of the divergence constrained at the discrete level is to apply a grad-div stabilization~\cite{MR3561143}: we add $\bm 0 = -\delta \nabla \dive \u$, with $\delta=\mathcal O(1)$, to the first equation of~\eqref{prob:cont}. In variational form, this is equivalent to add $\delta \int_\Omega \dive \u_h \dive\vv_h$ to the left-hand side of~\eqref{cutfem:disc_pb_nonsym}. From Figures~\ref{figure:div_plate3},~\ref{figure:div_plate4} we observe the positive effects of the grad-div stabilization.

\begin{figure}[!ht]
	\centering
	\subfloat[Without stabilizations.]
	{
			\includegraphics[width=0.33\textwidth,keepaspectratio=true]{div_plate_nostab}  \label{figure:div_plate1}
	}
	\subfloat[With ghost penalty.]
	{
		\includegraphics[width=0.33\textwidth,keepaspectratio=true]{div_plate_stab} \label{figure:div_plate2}
	}\\
	\subfloat[With ghost penalty, grad-div\\ and $\delta=100$.]
{
	\includegraphics[width=0.33\textwidth,keepaspectratio=true]{div_plate_graddiv_100}  \label{figure:div_plate3}
}
	\subfloat[With ghost penalty, grad-div\\ and $\delta=1000$.]
{
	\includegraphics[width=0.33\textwidth,keepaspectratio=true]{div_plate_graddiv_1000} \label{figure:div_plate4}
}
	\caption{\emph{$\dive\u_h$ in the square with circular trimming} obtained with~\eqref{cutfem:disc_pb_nonsym}.}\label{figure:div_plate}
\end{figure}
